Efficient DNN-Powered Software with Fair Sparse Models

With the emergence of the Software 3.0 era, there is a growing trend of compressing and integrating large models into software systems, with significant societal implications. Regrettably, in numerous instances, model compression techniques impact the fairness performance of these models and thus the ethical behavior of DNN-powered software. One of the most notable example is the Lottery Ticket Hypothesis (LTH), a prevailing model pruning approach. This paper demonstrates that fairness issue of LTHbased pruning arises from both its subnetwork selection and training procedures, highlighting the inadequacy of existing remedies. To address this, we propose a novel pruning framework, Ballot, which employs a novel conflict-detection-based subnetwork selection to find accurate and fair subnetworks, coupled with a refined training process to attain a high-performance model, thereby improving the fairness of DNN-powered software. By means of this procedure, Ballot improves the fairness of pruning by 38.00%, 33.91%, 17.96%, and 35.82% compared to state-of-the-art baselines, namely Magnitude Pruning, Standard LTH, SafeCompress, and FairScratch respectively, based on our evaluation of five popular datasets and three widely used models. Our code is available at https://anonymous.4open.science/r/Ballot-506E.

==> trash/Background.tex <==
\section{Background}\label{sec:bg}
\jwp{Overall version. I need to refine it.}
\subsection{Pruning}

% Network pruning is an important technique for reducing memory size and bandwidth usage.
% % Pruning techniques were first introduced in the early 1990s to shrink a large trained network into a smaller one, eliminating the need for retraining~\cite{lecunOptimalBrainDamage1989}.
% Researchers have proposed different methods to prune weights, neurons, blocks, as well as layers.
% By removing unnecessary elements of a network, pruning reduces the model size and increases the inference speed.

% In addition to reducing the model size, pruning presents an opportunity to improve the performance~\cite{wuFairPruneAchievingFairness2022} and generalization of the model.
Model pruning has emerged as a promising approach to address the scalability and efficiency issues associated with large neural networks. 
Pruning aims to reduce the model's size and computational burden while maintaining its performance by eliminating redundant or less critical parameters.
At its core, model pruning involves the selective removal of connections or neurons from the neural network. 
By identifying and removing the least influential or redundant weights or neurons, pruning seeks to create a more compact and lightweight model that can be deployed on memory-limited hardware without sacrificing accuracy.
Researchers have proposed different methods to prune weights, neurons, blocks, as well as layers~\cite{}.
By removing unnecessary elements of a network, pruning reduces the model size and increases the inference speed.
By retraining or fine-tuning the pruned model, it is possible to achieve a performance close to that of the original large model, and possibly the pruned model can even achieve better performance or generalization~\cite{}.
% In addition to reducing the model size, pruning presents an opportunity to improve the performance~\cite{wuFairPruneAchievingFairness2022} and generalization of the model.

% Furthermore, if pruned networks are retrained, it presents an opportunity to have a better performance~\cite{wuFairPruneAchievingFairness2022}.

% Add a figure
% Formally define.

\subsection{Lottery Ticket Hypothesis}
A recently proposed technique known as the Lottery Tickets Hypothesis~(LTH) has emerged as a rapidly growing field of study, which focuses on sparse trainable subnetworks within fully dense networks~\cite{frankleLotteryTicketHypothesis2018}.
% The lottery ticket hypothesis is a special case of network pruning, where the dense network is trained from scratch and the sparse subnetwork is trained from the dense network.
The LTH predicts that in a randomly initialized dense neural network, there exists a sparse initialized subnetwork that can achieve similar testing accuracy when trained independently for at most the same number of iterations.
These sparse neural networks, referred to as ``winning tickets''.
% Given a dense neural network $f(\theta)$ parameterized by $\theta$, the LTH states that there exists a sparse subnetwork $f(\theta_{0} \odot  m)$
Formally, for a randomly initialized dense neural network $f(\theta_{0})$ parameterized by $\theta_{0} \in \mathbb{R}^d$, LTH suggests searching a mask $m \in (\{0,1\}^d)$, i.e., the winning ticket is the sparse subnetwork $f(\theta_{0} \odot  m)$, where $\odot$ denotes the element-wise product. 
To find a winning ticket, it is common practice to first train the initialized network for some epochs and compute a mask based on the behaviors of the trained model.
LTH-based pruning usually follows the ``train-prune-retrain'' pipeline as shown in \autoref{fig:overview}.
Given a dense neural network \(f(\theta_{0})\) initialized by the parameter \(\theta \in \mathbb{R}^d\) and the pruning rate \(p\%\), the process of finding a lottery ticket can be expressed as: 
\begin{enumerate}
\item[i)] Train the network \(f(\theta_{0})\) for some epochs to get a well trained model \(f(\theta)\).
\item[ii)] Prune \(p\%\) of the parameters in \(\theta\) and creating a mask \(m \in (\{0,1\}^d)\).
\item[iii)] Reset the remaining parameters to their initial values in \(\theta_{0}\), creating the winning ticket \(f(\theta_{0} \odot  m)\).
\item[iv)] Train the winning ticket \(f(\theta_{0} \odot  m)\) to get final pruned model \(f(\theta^{*})\).
\end{enumerate}
\jwp{Maybe need to alignment the procedure with the Overview figure. \& Fix formatting problems with item numbers}
% \begin{enumerate}[label=(\roman*)]
%     \item Train the network \(f(\theta_{0})\) for some epochs to get a well trained model \(f(\theta)\).
%     \item Prune \(p\%\) of the parameters in \(\theta\) and creating a mask \(m \in (\{0,1\}^d)\).
%     \item Reset the remaining parameters to their initial values in \(\theta_{0}\), creating the winning ticket \(f(\theta_{0} \odot  m)\).
%     \item Train the winning ticket \(f(\theta_{0} \odot  m)\) to get final pruned model \(f(\theta^{*})\).
% \end{enumerate}
With the LTH-based pruning, it can produce a sparse model \(f(\theta^{*})\), which usually satisfies the performance requirement:
\begin{equation}\label{eq:pruneperformance}
    Acc(f(\theta)) - Acc(f(\theta^{*})) <= \epsilon
\end{equation}
where the \(\epsilon\) is the tolerable decline in test accuracy from pruning.
It is worth mentioning, although LTH presents the optimal winning tickets that exist in theory, how to perform the ticket selection remains an open problem.



% More formally, 
% Given a dense neural network $f(\theta)$ parameterized by $\theta \in \mathbb{R}^d$,
% there exists a binary mask $m \in (\{0,1\}^d)$ which lead to a winning ticket $f(\theta \odot m)$, where $\odot$ denotes the element-wise product.







\subsection{Fairness of Pruning}

The fairness of ML systems is a widely discussed problem.
In this paper, we focus on the following two metrics to measure the fairness of a classification model:

\smallskip
\noindent \textbf{Class-wise Variance~(CWV)~\cite{tianAnalysisApplicationsClasswise2021}.}
Given a dataset with \(C\) classes and the model accuracy \(a_{c}\) for each class \(c\), CWV can be defined as:
\begin{equation}\label{eq:cwv}
    \text{CV} = \frac{1}{|C|} \sum_{c\in C} ( a_c - \bar{a} )^2,\; 
    \bar{a}=\frac{1}{|C|}\sum_{c\in C} a_c
\vspace{-6pt}
\end{equation}

\smallskip
\noindent \textbf{Maximum Class-wise Discrepancy~(MCD)~\cite{tianAnalysisApplicationsClasswise2021}.}
For a model, given the maximum and minimum class accuracy \(a_{max}\) and \(a_{min}\), MCD can be defined as:
\begin{equation}\label{eq:MCD}
    \text{MCD} = a_{\max}-a_{\min}
\vspace{-4pt}
\end{equation}

Intuitively, CWV measures the average discrepancy, and MCD
uses the extreme discrepancy among classes, to estimate the fairness of a given model. 
The larger these values are, the more biased the given model is.
A fair pruning technique requires that the fairness metrics of the sparse model after pruning should not deteriorate significantly compared to the original model before pruning.
Formally, for a original model \(f(\theta)\) and a pruned model \(f(\theta^*)\), the fairness criterion can be defined as:
\begin{equation}\label{eq:prunefairness}
    d(f(\theta ^ *)) - d(f(\theta)) <= \delta
\end{equation}
where \(d\in\{CV, MCD\}\) computes the fairness metric, and \(\delta\) is the fairness tolerance.
If the criterion is not satisfied, we consider the pruning process to have a \textit{fairness bug}.


Previous work has demonstrated that pruning typically inherits or even amplifies fairness issues while reducing the model size~\cite{}. 
\jwp{Maybe give an example as given in ``Ciliate''}
